Distributed Inertial Best-Response Dynamics

The note considers the problem of computing pure Nash equilibrium (NE) strategies in distributed (i.e., network-based) settings. The paper studies a class of inertial best response dynamics based on the fictitious play (FP) algorithm. It is shown that inertial best response dynamics are robust to informational limitations common in distributed settings. Fully distributed variants of FP with inertia and joint strategy FP with inertia are developed and convergence is proven to the set of pure NE. The distributed algorithms rely on consensus methods. Results are validated using numerical simulations.

==> problem_setup_old.tex <==
% !TEX root = dfp_inertia.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Preliminaries} \label{sec_prelims}
A game in normal form is represented by the tuple $\Gamma := (\calN,(\calA_i,u_i)_{i\in \calN})$, where $\calN = \{1,\ldots,n\}$ denotes the set of players, $\calA_i$ denotes the finite set of actions available to player $i$, and $u_i:\prod_{i\in \calN}\calA_i \rightarrow \mathbb{R}$ denotes the utility function of player $i$. Denote by $\calA:= \prod_{i\in \calN} \calA_i$ the joint action space.

We suppose players are permitted to use probabilistic strategies. Formally, let the \emph{mixed strategy space} of player $i$ be given by the set $\triangle(\calA_i)$ of probability distributions over $\calA_i$, and let $\triangle^n(\calA):=\prod_{i=1}^n \triangle(\calA_i)$ denote the set of joint mixed strategies where it is assumed that players use independent strategies. We represent a joint mixed strategy $\sigma\in\triangle^n(\calA)$ as the $n$-tuple $\sigma = (\sigma_1,\ldots,\sigma_n)$, where $\sigma_i\in\triangle(\calA_i)$ denotes the marginal mixed strategy of player $i$. When a mixed strategy $\sigma\in\triangle^n(\calA)$ is played, we are interested in the expected payoff which, in a slight abuse of notation, we write as
%In an abuse of notation, the expected utility of player $i$ given the mixed strategy $\sigma\in \Delta$ is denoted by
%\vskip-5pt
\begin{equation}
\label{def_mixed_U}
U_i(\sigma) := \sum_{a \in \calA} u_i(\sigma)\sigma_1(a_1)\ldots \sigma_n(a_n)
\end{equation}
\vskip-5pt
The notation $u_i(\sigma_i,\sigma_{-i})$ is meant to emphasize that the payoff depends on the strategy $\sigma_i$ chosen by player $i$ and the strategies $\sigma_{-i}:=\{\sigma_j\}_{j\in\calN\backslash\{i\}}$ that are chosen by other players.

Given a strategy $\sigma_{-i}\in \prod_{j\in\calN\backslash\{i\}} \triangle(\calA_i)$, the \emph{best response} set of player $i$ is given by $BR_i(\sigma_{-i}):=\arg\max_{\sigma_i\in\triangle(\calA_i)} u_i(\sigma_i,\sigma_{-i})$. 
A mixed strategy $\sigma\in\triangle^n(\calA)$ is said to be a \emph{Nash equilibrium} if $\sigma_i \in BR(\sigma_{-i})$ for all $i\in\calN$. 
%$u_i(\sigma_i,\sigma_{-i}) \geq u_i(\sigma_i',\sigma_{-i})$ for all $i\in\calN$ and $\sigma_i'\in\triangle(\calA_i)$.

%\subsection{Repeated Play}
The learning algorithms considered in this paper assume the following format of repeated play. Let a normal form game $\Gamma$ be fixed. Let players repeatedly face off in the game $\Gamma$, and for $t\in\{1,2,\ldots\}$, let $a_{i,t}\in \calA_i$ denote the action played by player $i$ in round $t$. Let the $n$-tuple $a_t = (a_{1,t},\ldots,a_{n,t})$ denote the joint action at time $t$.

In this note we will be interested in algorithms for computing NE in a distributed information setup. We will say an algorithm is distributed if it satisfies the following assumption.\footnote{NOTE: This feels like a strange place to put this assumption since we're not actually dealing with distributed stuff until later in the paper. We could put it in it's own section before the section on distributed FP, but it seems too small a thing for a section (especially since the note needs to be short). Or we could introduce it in Section IV with distributed FP. But the central idea of our paper is developing algorithms for a distributed framework. So it seems strange to introduce is in a subsection late in the paper. So this felt like a reasonable compromise.}
\begin{assumption} \label{a_comm_graph}
Players are equipped with a pre-assigned, possibly sparse, communication graph $G=(\mathcal{V},\mathcal{E})$, in which a vertex represents a player, and an edge from vertex $i$ to $j$ represents the ability of player $i$ to communicate information to player $j$. The directed graph $G$ is strongly connected. Players may exchange information with immediate neighbors (the set of neighbors of a player $i$ is given by $\calN_i := \{j\in\calN:(i,j) \in \calE\}$) once between iterations of the repeated play process.
\end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Best-Response Dynamics} \label{sec_repeated_game_play}

Suppose that players are engaged in repeated play of some game $\Gamma$ and that prior to round $t$, each agent $i$ forms an estimate $\hat \sigma_{-i,t}^i$ of the mixed strategy $\sigma_{-i,t}$ that will be used by other agents in the upcoming round. The estimated strategy $\hat \sigma_{-i,t}^i$ allows agent $i$ to estimate the payoff that it would receive from playing an arbitrary action $a_i\in\calA_i$. These estimated payoffs can be written as
%
\begin{equation} \label{eqn_estimated_utility}
   \bru_{i,t}(a_i):= u(a_i, \brsigma_{-i,t}^{i}),~~ a_i\in \calA_i.
\end{equation}
%
In a best response learning algorithm, in each stage of the repeated play, each player plays an action that maximizes her utility given her estimate of the strategies of others.

In this paper, we are interested in a slight modification in which agents are sometimes ``reluctant'' to modify their action choices from round to round. We refer to this general algorithm (formally stated next) as \emph{inertial best response dynamics}.\footnote{We also refer to an algorithm of this form as an inertial best response algorithm.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}\label{algo_fp_inertia} \normalfont
Let $\rho\in (0,1)$ be an inertia constant and let $a_{i,1}$ be an arbitrary initial action for each $i$. At time $t>1$, agent $i$ has access to strategy estimates $\brsigma_{j,t}^{i}$ and a belief $\mu_{i,t}$ that it uses to compute the best response set $BR(\hat \sigma_{-i,t}^i)$.
%$\bra_{i,t}$ in \eqref{eqn_br_to_estimated_utility}.
Players are said to follow inertial best response dynamics if they play actions according to
%
\begin{equation}\label{eqn_def_inertia}
   \mathbb{P}\left(a_{i,t+1} = a_{i,t}\vert \mathcal{F}_{t-1}\right) = \rho, \quad
   \mathbb{P}\left(a_{i,t+1} \in \bra_{i,t}\vert \mathcal{F}_{t-1}\right) = 1 - \rho,
\end{equation}
\end{algorithm}
where $(\mathcal{F}_t)_{t\geq 1}$ is a filtration (sequence of increasing $\sigma$-algebras) that contains the information available to players in round $t$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
As per \eqref{eqn_def_inertia}, an inertial best response algorithm entails player $i$ sticking to its previous play $a_{i,t}$ with some (fixed) probability $\rho$ (this is the inertia component of the algorithm), and playing a best response otherwise.
%The selection of myopic best responses promotes a general trend of improving utility, while the inertia component of the algorithm---with its occasional repetition of actions---ensures that players eventually lock into a pure strategy equilibrium. Examples of algorithms that use best response with inertia can be found in \cite{Young_2004, Marden_et_al_2009}.

%Throughout this paper, we want to study mechanisms to update the beliefs $\brsigma_{j,t}^{i}$ so that players learn pure equilibria (cf. Definition \ref{def_equilibria}). We do so using ideas from fictitious play, so that (roughly speaking) $\brsigma_{j,t}^{i}$ is built from empirical histograms of the actions that have been observed or action information that has been disseminated through an overlaid communication graph. These algorithms are defined in Sections \ref{sec_D-FP} and \ref{sec_D-JSFP} after we introduce some preliminary convergence results for the generic inertial best response methods given in Algorithm \ref{algo_fp_inertia}.

\subsection{General Assumptions}
Unless otherwise specified, throughout the paper we will consider inertial best response dynamics in games satisfying the following assumptions.
\begin{assumption} \label{a_acyclic_game}
The game $\Gamma$ is weakly acyclic.
\end{assumption}
\begin{assumption} \label{distinct_actions_assumption}
For any pair of actions $a_i',a_i'' \in\calA_i$, $a_i'\not=a_i''$ and for any $a_{-i}\in\calA_{-i}$,
$$
u_i(a_i',a_{-i}) \not= u_i(a_i'',a_{-i}).
$$
\end{assumption}
We remark that Assumption 3 is generic in the sense that
if the number of players and actions are fixed, then the set
of utility functions for which Assumption 3 fails is a closed
set of Lebesgue measure zero within the space of all possible
utility functions.
\begin{assumption}\label{a_measurability}
%Let $H_{t} := \{a_s\}_{s=1}^t$ denote the action history through round $t$.
Let $\{\mathcal{F}_{t}\}_{t\geq 1}$ be a filtration (sequence of increasing $\sigma$-algebras) with $\mathcal{F}_{t} := \sigma(\{a_s\}_{s=1}^t)$.
The strategy estimate $\hat \sigma_{j,t}^{i}\in\triangle(\calA_j)$ that agent $i$ has of the strategy $\sigma_{j,t}$ of agent $j$ is measurable with respect to $\mathcal{F}_t$.
\end{assumption}

Assumption \ref{a_measurability} means that the strategy estimates of agent $i$ are restricted to be a function of the history of play.

